Explorative Data Analysis for Changes in Neural Activity

Neural recordings are nonstationary time series, i.e. their properties typically change over time. Identifying specific changes, e.g. those induced by a learning task, can shed light on the underlying neural processes. However, such changes of interest are often masked by strong unrelated changes, which can be of physiological origin or due to measurement artifacts. We propose a novel algorithm for disentangling such different causes of non-stationarity and in this manner enable better neurophysiological interpretation for a wider set of experimental paradigms. A key ingredient is the repeated application of Stationary Subspace Analysis (SSA) using different temporal scales. The usefulness of our explorative approach is demonstrated in simulations, theory and EEG experiments with 80 Brain-Computer-Interfacing (BCI) subjects.

==> sec03_simulations.tex <==
% !TEX root = Subprojection.tex 

\section{Simulations on Synthetic Data}
\label{sec:simulations}

In this section, we evaluate the proposed method in controlled simulations on synthetic 
data, where we can objectively assess the performance based on an artificial ground truth.
Our analysis consists of two parts. First of all, we investigate how accurately our algorithm 
can identify the true condition-shared stationary components. In our model, these are the 
relevant components for subsequent analysis. In the second part of this section, we show 
that these components are useful. To that end, we apply our method as a pre-processing step to 
change-point detection in a situation where there are irrelevant condition-shared non-stationary 
components, which we want to remove. We analyse the relative merits of our pre-processing 
in different scenarios.

\subsection{Data Generation}
\label{sec:data}

The synthetic data that we use in the controlled simulations is generated according to our 
model (Equation~\ref{eq:model}). At each time point, the observed $D$-variate sample $x_k(t)$ 
in the $k$-th condition is a sum of contributions from the condition-shared and the 
condition-specific system. The condition-shared variables are linearly transformed by a 
random orthogonal mixing matrix $A \in \R^{D \times D}$ that is kept fixed over all conditions. 
The condition-specific components are linearly transformed by an orthogonal mixing matrix 
$B_k \in \R^{D \times D}$ that is chosen randomly for each condition $1 \leq k \leq K$, where 
$K$ is the total number of conditions. In the simulations, the number of stationary and 
non-stationary components is kept fixed for both systems.

The condition-shared and the condition-specific system each comprises
two groups of components: stationary and non-stationary. The mean and
covariance matrix of the stationary components are the zero vector $0$
and the identity $I$ respectively. The mean of the non-stationary
components is also fixed to zero, whereas the covariance matrix is
chosen according to two Markov models, one for the condition-shared
and one for the condition-specific system. Both Markov models consists
of five states corresponding to five covariance matrices. The
covariance matrices are diagonal with entries drawn randomly
random from a set of log-spaced values over the intervals $(1, \nu)$ and $(1/\nu, 1)$ with $\nu >
1$; thus a high $\nu$ corresponds to a high level of non-stationarity. For the condition-shared system, this parameter is
$\nu_\text{shared}$ and for the condition-specific it is
$\nu_\text{specific}$.  The probability of changing the state in the Markov model
(i.e.\ switching to another covariance matrix) is parametrized by
$p_\text{shared}$ and $p_\text{specific}$ for the condition-shared and
the condition-specific system respectively. Thus a low $p$ corresponds to few changes occurring. The shortest segment of stationary data possible consists of $50$
samples, generated from a Gaussian with the respective covariance
matrix; thus changes may occur at most once every 50 data points.

To sum up, the key parameters of interest are the strength of the non-stationarity in both
systems ($\nu_\text{shared}$ and $\nu_\text{specific}$), and the probability of changes in the
covariance matrix of the non-stationary sources ($p_\text{shared}$ and $p_\text{specific}$). 

%% OLD TEXT BELOW 
%Each of these subsystems is generated as a linear mixture of stationary and non-stationary sources. We denote the subsystem, either condition-specific or condition-shared by $\theta$, with $\theta =$ "condition shared" or "condition-specific". The non-stationary data is further generated time segment wise: each segment has fixed 
%length (for example each segment may be 50 data points in length) and each dataset consists of a concatenation of time segments\footnote{Note the difference here between ``time segment" and ``epoch"; ``time segment" refers to a section of data, which according to the generative model for the synthetic data setup, is stationary, whereas we use ``epoch" to denote a length of data chosen to calculate sample covariances and means for the purpose of the SSA computations.}.
%
%The $d_s^\theta$ stationary sources are distributed normally on each time segment according to $\mathcal{N}(0,I_{d_s^\theta})$. The other $d_n^\theta$ (non-stationary) source signals $s^n(t)$ are distributed according to the active model $k$ of this time segment; this active model is one of five Gaussian distributions $\mathcal{G}_k = \mathcal{N}(0,\Sigma_k)$: the covariance $\Sigma_k$ is a diagonal matrix whose eigenvalues are chosen at random from five log-spaced values between $\sigma_1^2 = 1/p_\theta$ and $\sigma_5^2 = p_\theta$; thus five covariances, corresponding to the $\mathcal{G}_k$ of the Markov chain are then chosen in this way. The transition between models over consecutive time segments follows a Markov model with transition probabilities:
%\begin{equation}
%	P_{ij} = 
%	\begin{cases} 
%		1-t_\theta   & i=j \\ 
%	         t_\theta/5 & i\neq j .
%	\end{cases}	
%\end{equation} 
%
%Thus, the parameter $t_\theta$ controls the probability of changes in each system, and the parameter $p_\theta$ controls the strength of the changes.
%Note that for each condition and subsystem, the setup is identical to the setup studied in \cite{blybunmeimul12feature}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Finding the Condition-Shared Stationary Sources}
\label{sec:get_pub}

In the first set of experiments, we investigate how well our method can identify the true stationary
components of the condition-shared system. We analyze the influence of the number of different conditions 
in two scenarios: low and high condition-specific degree of non-stationarity. 
The total number of dimensions is set to 20 and the number of non-stationary directions is set to 
1 and 2 for the condition-specific and condition-shared system respectively; the total number of samples
is 10000. The error is measured as the subspace angle between the true non-stationary subspace
of the condition-shared system and the estimated one. 

\begin{figure}
	\centering
	\includegraphics[width=120mm]{performance_int.pdf}
	\caption{
	Performance of the proposed method measured in terms the subspace angle (vertical axis) between the true
	and the estimated non-stationary subspace of the condition-shared system, for different numbers 
	of conditions (horizontal axis). The left and right panels shows the results for the cases where the
	condition-specific non-stationarity is low and high respectively.
%	The figure displays results showing how accurately SSA may be used to identify the shared stationary subspace. The simulation setup is described in Section~\ref{sec:get_pub}, where we evaluate the performance of SSA in obtaining the condition-shared stationary projection. In both plots, the quantities on the $x$-axis denote the number of conditions. The figure displays on the left a low degree of power change ($q_\text{power} = 1.8$) in the individual condition systems whereas on the right a high degree ($q_\text{power} = 3.0$). In each case, the red line denotes the case in which the condition-specific systems are replaced with stationary noise $d_k = D$ as a baseline result. The red line case thus represents the limit in potential accuracy
%possible for the blue line, which represents the accuracy for the case in which the condition-specific systems contain significant non-stationary contributions. In the low degree power case, the condition-specific systems make little
%contribution to the error, whereas in the high degree this is not the case. However, in the high degree case, the error
%decreases with the number of conditions.
\label{fig:acc_sim}
}
\end{figure}

The results are shown in Figure~\ref{fig:acc_sim}. In the left panel, we see the results for low 
condition-specific non-stationarity. As we increase the number of conditions, the error of finding the 
true stationary components (blue line) becomes smaller. This is because the non-stationary contributions of the 
condition-specific systems become more equally spread across the whole $D$-dimensional space since for 
every condition $k$ we choose a random mixing matrix $B_k$. This allows us to distinguish more clearly 
between the condition-shared and the condition-specific non-stationary directions and, in turn, find 
the condition-shared stationary components. The red line shows the error on the same data where we 
have removed the condition-specific contributions: this is the lowest possible error level on the condition specific model for finite samples. We see that as soon as we have at least four different conditions, 
we can identify the true condition-shared stationary components as well as if there were no 
condition-specific non-stationarities.

The right panel shows the results in the case where the degree of non-stationarity in the condition-specific 
system is high relative to the condition-shared system. As we can see, this makes the desired stationary components 
of the condition-shared system more difficult to identify than in the previous case, because the 
overall distribution is dominated by changes in the condition-specific system. We therefore need a larger number 
of conditions (around 11) in order to distinguish between the non-stationarity of the two systems. 

%The aim in this section is to assess the quality of the approach outlined in Section~\ref{sec:public_method}, i.e. using SSA to obtain a projection to the publicly stationary directions $\hat P_0$.
%
%We set the number of dimensions to $D=20$ and the number of pooled system stationary dimensions to $d^*=18$. For each condition we set the number of stationary dimensions in the condition specific system to $d_k = 19$ for all $k$.
%The number of data points is set to $10,000$ and orthogonal mixing matrices are chosen for each system of the same magnitude. We then vary the number of conditions $K$ from 1 to 20 for various values of the power change $q_\text{power}$ in the condition-specific non-stationary sources
%while keeping the power change in the condition general system at $2.3$ and for all realizations of the dataset we compute the angle between the calculated subspace and the genuine subspace. To assess the quality of the result, we compare the accuracy on the setup described with the accuracy on a time series of the same type, but where each of the condition specific
%systems is replaced by stationary noise.
%
%The results are displayed in Figure~\ref{fig:acc_sim}. 
%%\textbf{PB: description and interpretation of results is missing due to missing figure.}
%One observes that when the power change in the condition-specific systems is low, then the accuracy of SSA is not affected by the additional non-stationarities.
%However, as the power change grows, few conditions implies lower accuracy. However, even for power change $q_\text{power}$ higher than $2.3$, the accuracy is recovered given enough conditions.



%\subsection{Hypothesis Testing Between Two Classes}
%
%\label{sec:hyp_test}
%
%In this section we assume that 
%\begin{equation}
%\mathcal{L}_{D}(B_1^k,\dots,B_i^k,\dots,B_1^k)) > \mathcal{L}_{D}(B_1^k\dots,B^{k'}_i,\dots,B_1^k)
%\end{equation}
%We then investigate the change in the testing errors when confining the test to an estimate of the projection of the data by $P_0$. We show 
%that when the number $d^*$ is high, then the increase in testing error is negligible, taken over random experiments.
%We take the same setup as above, described in Section~\ref{sec:get_public} but keeping the number of classes constant and varying $d^*$, the number
%of stationary directions in the class-sharedsystem. The results are displayed in Figure~\ref{fig:hyp_sim}. This time we take the number of dimensions, $D = 20$, the number of class-specific
%stationary directions $d_k = 19$ for each $k$. For the first class involved in the test we take $q_\text{power} = 1.5$, for the second, $q_\text{power} = 20$. We take $q_\text{power} = 2.5$ for
%the class-sharedsystem. In addition, we take the number of classes as $K = 9$. We then vary $d^*$, the number of publicly stationary directions from $1$ to 19.
%
%The results show that if the number of public, non-stationary directions is not too high, then the decrease in testing power obtained when confining
%a test to the estimated publicly stationary directions is low. Of course, when the number of publicly non-stationary directions is too high, then 
%the testing error increases.
%
%\begin{figure}
%\begin{center}
%\includegraphics[width=90mm]{testing.pdf} 
%\caption{The figure displays the results from the simulation described in Section~\ref{sec:hyp_test}. The $x-$axis displays the value of $d$-star, the number of public, stationary directions. The $y$-axis displays the probability that the non-stationary error in one class's distribution is greater than the error measured on the orthogonal complement to the class
%pooled non-stationarity: that is to say, the probability that we reject the hypothesis that the two classes have the same level of non-stationarity. 
%The red line displays the mean error in testing this hypothesis when $d^star = D$, i.e. there are no class-sharednon-stationary directions. 
%The green line displays the mean error if the fact projection to the pooled stationary directions is obtainable, whereas the blue 
%line displays the mean error if this projection is estimated. 
%Thus, the results show that when the number of pooled non-stationary directions is low, then the increase in error is small and 
%the extra error incurred by estimation of the projection is not large.
% \label{fig:hyp_sim}}
% \end{center}
%\end{figure}

\subsection{Identification of the Background Non-Stationary Components in Simulated EEG}

We illustrate the application of SSA to artificial data generated by a
realistic EEG forward model.
% Do I need background here?
%to simulate an EEG recording where the model is applicable. 
The head model we use was calculated on the basis of the MRI scans of
152 human participants \cite{Kopfmodel1}, the electrodes were placed
on the head according to the international 10-5 system and the
forwards mapping from simulated dipoles to voltages at the electrodes
were computed using the semi-analytic methods of the contribution of
Nolte et al. \cite{LeadFields}.
%; this model and method have been studied in numerous contributions in the 
%neuroscientific literature \cite{PSI,}
Given this framework we simulated two background non-stationary
sources, the first 2 cm underneath the electrode T7 close to the edge of the montage, to simulate the effects of a non-stationary 
EMG component and the second at the primary 
visual cortex, 2cm under the electrode Oz, to simulate the effect of a non-stationary alpha source. 


Subsequently we modeled three scenarios.
In the first scenario, for each of 13 conditions, in addition to the two background non-stationary sources, a non-stationary source was positioned
at random in the brain together with 12 stationary sources, thus the dataset has dimensionality 15, within a 118 (the number of electrodes) dimensional space. The non-stationarities were generated using a Markov model, giving rise to segments of simulated EEG data 
with varying power.
We computed the estimated background non-stationary components using SSA 
and the estimated condition specific components, for the first 2 conditions.
The results of this first scenario are displayed in Figure~\ref{fig:ForwardModel} and show that SSA successfully locates the EMG and alpha component, and succeeds in obtaining asymmetric non-stationary components between the first two
classes, which match the true non-stationary condition specific patterns. Moreover, we see that using SSA separately on each class does not deliver the background non-stationarities and the condition specific non-stationarities successfully, whereas estimation of the background non-stationarities over conditions using SSA is successful as described in Section~\ref{sec:public_method}, following which the condition specific non-stationary patterns are successfully
found. 

Although, in general the background non-stationarities may only be reliably obtained given many conditions, we may still consider whether using SSA to remove background non-stationarities works
when we have only two conditions and under which circumstances. Thus, in the second scenario, we reduce the number of conditions to two and simulate background non-stationary sources which are \emph{stronger}
in their non-stationarity than the condition specific non-stationary sources. All other settings are kept constant. The results of this second scenario are displayed in Figure~\ref{fig:ForwardModelTwoClasses}
and show that in this case, when the background non-stationarities are strong, then these, and subsequently the condition specific non-stationarities, may be obtained nonetheless, using the proposed method.

However, in the third and final scenario we see that when the number of conditions is two and the condition specific non-stationarities are weak, then obtaining patterns using SSA on each condition separately which
nevertheless agree across the conditions, and thus may be assumed to correspond to background non-stationarities, occurs only after the most non-stationary components have been removed. The results of this third
scenario are displayed in Figure~\ref{fig:ForwardModelSpike}.
We will
see, in the analysis of the BCI data in Section~\ref{sec:application}, that both of these second and third scenarios may arise.

\begin{figure}
\begin{centering}
\includegraphics[width=114mm,clip=true,trim=1mm 80mm 105mm 70mm]{ForwardModelScrew.pdf}
\caption{The figure displays scalp plots computed using SSA on the EEG forward model data. The left panel displays the true non-stationary patterns, and the right hand panel displays
the estimated condition specific non-stationary patterns after removal of zero, one and two background non-stationary directions. The plots show that SSA successfully obtains the patterns resulting
from the background non-stationary alpha and background non-stationary EMG, and then allows one to concentrate on the condition specific non-stationarities in each class. Note that
after removing one background non-stationary direction, SSA finds a difference between the conditions. This is because, for the two conditions studied, the condition specific non-stationarities
are strong. Nevertheless, SSA successfully obtains the correct background non-stationarity, so that the final condition specific non-stationarities are correct.
 \label{fig:ForwardModel}}
\end{centering}
\end{figure}

\begin{figure}[h]
\begin{center}$
\begin{array}{cc}
\includegraphics[width=152mm,clip=true,trim=1mm 87mm 10mm 80mm]{ForwardModelTwoClasses}\\
\end{array}$
\end{center}
\caption{The figure displays the results of the forward model simulation when the number of conditions is two and the background non-stationarities are 
stronger than the condition specific non-stationarities. Here, using SSA, one obtains the background stationarities as estimated "condition-specific" non-stationarities
which agree across conditions after zero and one background non-stationarities have been removed. The condition specific non-stationarities are then 
obtained after the removal of two background non-stationary directions.
\label{fig:ForwardModelTwoClasses}}
\end{figure}

\begin{figure}[h]
\begin{center}$
\begin{array}{cc}
\includegraphics[width=110mm,clip=true,trim=3mm 85mm 20mm 80mm]{SpikeInSpectrum}\\
\end{array}$
\end{center}
\caption{The figure displays the results of the forward model simulation when the number of conditions is two and the condition specific non-stationarities are 
stronger than the background non-stationarities. Here, after removal of zero, one and two background non-stationary directions, SSA finds \emph{different}
non-stationary patterns on each condition. However, after removal of three background non-stationary directions, SSA finds non-stationary patterns on each condition
which agree, and arise, in fact, from the true background non-stationarities. The reason that the condition specific non-stationarities are similar after removal of
zero and one background non-stationary directions, is because the first estimated \emph{background} non-stationary direction is nevertheless correct, 
the EMG component, so the condition specific most non-stationary directions are preserved. These are then removed as the estimated second and third most 
non-stationary background directions.
\label{fig:ForwardModelSpike}}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Application to Change-Point Detection}
\label{sec:cp_d}

In this section, we demonstrate that the proposed method can be used to find \textit{relevant} change-points 
in the data from a particular condition of interest, even when there are \textit{irrelevant} 
distribution changes that are shared by all conditions. In reality, this situation occurs e.g.\ when 
there are artifacts in the data that are independent of the experimental condition. 

Change point detection refers to the task of detecting points in time in which the distribution 
of a time series changes from one state to another; this task occurs potentially in sleep staging of 
EEG recordings \cite{switch_dynamics} and in early warning systems for epilepsy patients using chronically 
implanted electrodes \cite{Celka20021}, among other applications \cite{Speech1,Econ1,Econ2}. There
exists a wide range of different methods for change-point detection (also called time series segmentation). 
In our simulations, we use single linkage clustering based on a symmetrized Kullback-Leibler divergence 
measure~\cite{Gower69SingleLinkage,blybunmeimul12feature_DISCRIM} between segments of the time series. 

\begin{figure}[ht]
\begin{center}
\includegraphics[width = 120mm]{TempSegGridPlot}
%\begin{tabular}{c}
%\includegraphics[width = 125mm,height =28mm]{../experiments/exp_class_pooled/SQUARE_SIMULATION_MORE_NON_STAT.pdf} \\
%\includegraphics[width = 125mm,height =28mm]{../experiments/exp_class_pooled/SQUARE_SIMULATION_HIGH_TRANSITION.pdf}  \\
%\includegraphics[width = 125mm,height =28mm]{../experiments/exp_class_pooled/SQUARE_SIMULATION_IMBALANCE_TRANSITION.pdf} 
%\end{tabular}
\caption{
Results of the pre-processing for change point detection. The rows of the $3 \times 3$ grid 
correspond to three different scenarios: few condition-shared change points, many condition-shared change-points, and
few condition-specific changes but many condition-shared changes. From left to right, the columns 
shown the AUC without pre-processing (baseline), the AUC with pre-processing and a comparison
between the two (improvement). In each panel, we vary the strength of the condition-shared 
non-stationarity along the horizontal axis, and the strength of the condition-specific 
non-stationarity along the vertical axis.
%The figure displays the change-point detection simulation results. The red end of the color spectrum indicates high performance, whereas the blue end, poor performance. In each figure, the $x$-axis
%corresponds to the power in the condition-specific system and the $y$-axis corresponds to the power in the 
%condition-shared system. In each row, the left hand panel corresponds to the ratio in the mean performance between
%the case in which one performs change-point detection on the data without preprocessing and 
%the case in which one performs change-point detection on the data projected with the estimate public
%stationary projection; the middle panel in each row corresponds to the mean AUC values achieved on the data without preprocessing;
%the right hand panel in each row corresponds to the mean AUC achieved on the data projected with the estimate public
%stationary projection.
%In each case $D = 10$, $d_k=5$, $K = 10$. In the top row the transition probabilities are $\Gamma_c = 0.9, \Gamma_p = 0.9$. In the second 
%row, $\Gamma_c = 0.7, \Gamma_p = 0.7$ and in the bottom row $\Gamma_c = 0.1, \Gamma_p = 0.8$.
%The results show that projecting helps more if changes in the condition-shared system are likely and above a certain threshold  and 
%that projection helps most when the probability of changes in the condition-shared system are more likely than those in the condition-specific system.
\label{fig:temp_seg_class}}
\end{center}
\end{figure}

Here, we test the hypothesis that the performance of 
change-point detection can benefit from removing non-stationary directions (feature extraction) that 
are not specific to the condition of interest. Thus we suggest a \emph{pre-processing} step which 
aims to boost the performance of change-point detection, when the model applies.
Previous work 
\cite{blybunmeimul12feature_DISCRIM} has shown that removing stationary directions in a pre-processing step 
improves the performance of change-point detection. Here, we go one step further and distinguish between 
relevant and irrelevant non-stationary changes by making use of data from other conditions 
during feature extraction to remove the background \emph{non-stationary changes}.The problem 
setting is illustrated in Figure~\ref{fig:TempSegIllusBack}; here we see that infrequent and weak condition specific
changes are masked by stronger and more frequent background changes. This renders difficult detecting
the condition specific changes reliably. The solution we propose is to project the data to the background stationary
sources.

\begin{figure}
\begin{centering}
\includegraphics[width= 130mm,clip=true,trim=30mm 160mm 10mm 15mm]{TempSegIllusBack}
\caption{The change point detection task is made more difficult when the change points of interest in the condition specific system (left) are masked by background change points (right). \label{fig:TempSegIllusBack}}
\end{centering}
\end{figure}


The synthetic data is generated as described in Section~\ref{sec:data}. The total number of dimensions
is 10, the number of conditions is 10 and the number of non-stationary directions is 2 and 1
for the condition-shared and the condition-specific systems. In the simulations, we vary
the strength of the non-stationarity in both systems ($\nu_\text{shared}$ and $\nu_\text{specific}$), 
the likelihood of the relevant change points in the condition of interest ($p_\text{specific}$), and the likelihood 
of irrelevant change points in the condition-shared system ($p_\text{shared}$). 

As a baseline, we directly apply the change-point detection algorithm to the data from the condition 
of interest and discard the remaining nine data sets. We compare this approach against the augmentation
of this algorithm by our pre-processing (feature extraction). More specifically, we apply SSA to 
estimate the nine most stationary components \textit{over all conditions} and then apply the change-point 
detection algorithm to these components on the data from the condition of interest. We measure the performance 
in terms of the area under the receiver-operator curve (AUC). 

%The algorithm
%computes distances between the distributions of the data in windows approximated as Gaussians
%and performs clustering using the measured distances.
%
%In this section we 
%use the same data setup as above, in Section~\ref{sec:data} but this time test the of an algorithm
%for change point detection for detecting changes in one of the selected condition-specific systems.
%
%
%To this end, we test the performance of a change point detection algorithm on the raw data from the fixed condition 
%against the performance of the same algorithm on the raw data from that condition projected 
%by the estimated condition-shared stationary projection. In particular, we test the performance for 
%various ratios between the probability of a change in the condition-shared system and the condition-specific systems.
%
%
%By way of background, it has already been shown in the non-stationarity literature that
%SSA can be used to obtain non-stationary directions in the change-point detection
%context and that may be used in this capacity to boost the performance of arbitrary change-point
%detection algorithms \cite{blybunmeimul12feature}. We also
%show here that the stationary projection may also be used to boost the performance of SSA when 
%the current model under investigation is relevant. 
%
%More precisely, we set the $q_\text{power} = 2.3$ for the condition-shared and condition-specific systems, the number of 
%dimensions $D = 10$, the number of conditions, $K = 10$, the number of time segments in the time series to 100 
%and the number of time points per condition, per segment to 200, the number of condition-shared stationary directions to $d^* = 8$,
%the number of condition stationary directions to $d_k = 9$. In the simulations we vary the stability of the condition-shared and condition-specific
%markov model $\Gamma_{c}$ and $\Gamma_p$. 

The results are shown in Figure~\ref{fig:temp_seg_class}. The right column of the $3 \times 3$ grid 
shows the improvement in AUC due to our pre-processing for three different scenarios. When there 
are few condition-shared irrelevant change points (top row) \emph{and} few condition specific change points, the performance of change-point detection is 
relatively unaffected, there is improvement using a preprocessing step only when the condition shared changes are pronounced enough
to yield reasonable estimation of the desired projection. 

In the second row the case in which there are many irrelevant condition-shared change points as well as many condition-specific change points of interest.
which interfere with the detection of the relevant change points in the conditions of interest.
Thus, in the middle panel of the right column, we see that the proposed pre-processing leads to a 
significant improvement in performance for almost all cases. However, when both systems have
low non-stationarity (bottom left corner of the panel), 
it is hard to identify the informative 
condition-shared stationary components; hence the performance does not increase. 

The last simulations whose results are displayed in the bottom row, confirm that it is the frequency
of the changes in the distracting condition \emph{shared} system which determine whether a high 
level of improvement is to be expected. Here, as in the second row, the frequency of condition-shared
changes is high and the frequency of the desired condition-\emph{specific} changes is low.
As in the second row, improvement is to be expected in all cases except the cases in which
the strength of the condition-shared changes are not sufficient to yield reliable estimation
of the shared stationary projection.

%
%The results show that
%when the probability of a change in the condition-shared system is higher than the probability in 
%the condition-specific system, then projecting yields an overall improvement in AUC, except
%for when the strength of the condition-shared non-stationarity is very high.
%
%However, this is not true if the probabilities of changes are similar in each subsystem and both are low.
%In this case, there are both a range of parameter settings where not projecting
%out the estimated condition-shared non-stationarity yields higher AUC performance as well
%as a range of settings where projecting yields higher AUC performance.
%
%


==> sec_theorybounds.tex <==
% !TEX root = Subprojection.tex 

\subsection{Theoretical Results}
\label{sec:con_proof}

In this section we describe a theoretical guarantee for the quality of the approach outlined in the previous 
section. The rather technical proof is deferred to Appendix~\ref{app:proofs}; here we focus on the intuitive 
interpretation of the result. 
In particular, we will prove in Proposition~\ref{prop:converge} that the covariances resulting from forming SSA epochs containing several conditions will converge to stationarity in the limit of the numbers of conditions and stationary dimensions.
This allows the SSA algorithm to identify the desired part of the background system, because the only remaining factor affecting estimation are then the small sample effects affecting SSA.

%% PB: The below text is more confusing than helpful; there is no need to describe what cannot be done. 
%% 
%
%The first point to note is that SSA is not consistent for the model assumed without additional assumptions. The following example shows why.
%Specify the number of Dimensions as $D=2$, the number of shared non-stationary directions to be $d^*=1$ and for each $k$, the number of condition specific non-stationary directions
%to also be $d_k =1$. If the changes in the parameters in the condition-specific non-stationarities are identical across conditions (identical parameters for the projections and identical shifts between epochs), then the algorithm described in the previous section fails. This is because the identical non-stationarities across conditions add together to produce an overall non-stationarity across classes which differs in its mixing matrix from the condition shared component.
%This shows that there can be no general consistency proof of the correctness of the approach, as the model currently stands. Fortunately, however, it is highly improbable that this situation should arise in practice. This is because
%if the conditions correspond to the data resulting from distinct underlying dynamical systems then the distribution over data in the separate conditions will be independent from one another, both in the profile of changing parameters over time and the projections to the non-stationary condition specific systems. 
%
%The aim of our method is to remove the non-stationary contributions from the background system, which are 
%considered irrelevant (e.g.\ artifactual), in order to be able to analyze the non-stationarities occurring 
%in a particular condition. This is achieved by estimating the projection to the stationary components 
%using SSA with a particular epoch setup that is aligned to the condition-trial structure of the data, as 
%illustrated in Figure~\ref{fig:epoch_illustration}. More specifically, the SSA epochs are formed chronologically 
%such that each epoch consists of one trial from each condition. This means that the empirical covariance matrix 
%of each SSA epoch is an estimate of the average covariance over conditions, at a certain point in time. Since 
%SSA minimizes the non-stationarity between these epochs, the found stationary components are stationary 
%w.r.t.\ temporal changes of the average distribution over all conditions. In other words, the found 
%stationary projections remove non-stationary contributions from the background system, and not from the 
%condition-specific system. 
%
%The ideal solution is the projection to the true stationary components of the background system, as this 
%would remove all irrelevant non-stationary contributions. The confounding factors in obtaining
%this stationary projection are the non-stationary components of the condition-specific systems; if SSA 
%is computed on the $k$-th condition, the estimate produced for the stationary projection will 
%project to estimated sources which balance condition specific and background non-stationarity to be minimal, which
%is not what we require. 
%
%Any estimation of the background stationary projection must therefore use the information from all conditions. The accuracy of estimation using SSA as described in Section~\ref{sec:model} depends in part on 
%how well changing covariance on the epochs chosen approximates the changing covariance in 
%the background system. The factors affecting this approximation are the number of data points available, the number of 
%conditions available, the numbers of background non-stationary directions, the numbers of condition specific 
%non-stationary directions, the strength of the non-stationarities in the non-stationary sources of both systems
%and the generative character of the non-stationarity. Our analysis focuses on the generative character of the non-stationarity, the numbers of conditions 
%and the number of condition specific stationary dimensions. This is because the number of data points is only important insofar as it is important for SSA, the strength of the non-stationarities
%do not affect the qualitative convergence properties and the background non-stationary directions only affect convergence as for the standard SSA.


%Next steps in the writing:
%\begin{enumerate}
%	\item Explain what makes the situation more difficult than the standard SSA setting; i.e.\ explain why 
%			the presence of the condition-specific contributions make it more difficult to identify the demixing
%			matrix of the background system. 
%	
%	\item Clearly list the factors that influence how well the ideal solution can be found (number of stationary and 
%			non-stationary components, etc.). 
%	
%	\item Say that in essence, how well SSA can find the desired stationary components depends on how much the 
%			objective function is distorted by condition-specific non-stationarities.
%						
%	\item In this section, we present a bound in terms of the above factors (see 2.), which shows that the 
%			distortion of the cost function converges to zero. 
%	
%	\item This shows that our approach is theoretically well justified. 
%	
%\end{enumerate}


 

%Whether we can find this depends on a number of 
%factors: the number of stationary and non-stationary components in the background and in the condition-specific 
%systems respectively, and the number of conditions and trials. 


%The gist of the proposition we prove here, is that if there are enough shared-stationary directions, the class-non-stationary subspaces are sampled uniformly (i.e. independently from one another) and no class non-stationarity affects the data disproportionately, then the algorithm finds approximately the correct shared stationary subspace. These are realistic assumptions; for example, in EEG analysis, often the class-shared non-stationarities correspond to movement or eye blink related activity which only affects a low dimensional subspace of the data. Moreover, 
%the class-specific non-stationarities often are properties of distinct underlying physical systems, which implies that the subspace of data space they affect may be treated as a sample from a uniformly distributed random variable. Finally, the assumption
%that no class affects the data disproportionately is realistic, as in applications the class-specific non-stationarities are hard to obtain precisely because there power is weaker than the strength of the shared non-stationarities.
%
%\begin{Prop}
%Assuming that the directions of the non-stationarities in each of the classes are sampled from a uniform distribution and that the non-stationarity is bounded over classes in the limit of classes then the algorithm given in Equation~\ref{eq:alg_pub} is correct in the limit of
%the number of stationary directions.
%\end{Prop}

%The gist of the proof is to show that if there are enough conditions then projecting the $\hat{H}_n$ with the condition shared stationary projection gives the desired loss in the limit of numbers of conditions. 
%
%In order to show this, one bounds the deviation of the actual average covariance over conditions $H_n = \frac{1}{K}\sum_{k=1}^K C_n^k$ on an epoch to the average actual average covariance over classes over epochs $\bar{H} = \frac{1}{N}\sum H_n$ on a particular projection using the assumption that no condition contributes disproportionately to the non-stationarity level; one thus obtains
%terms which converge to zero. Set $C_{i,k} = R_{i,k} + \Sigma_i$ where $R_{i,k}$ is the condition specific part of the covariance and $\Sigma_i$ is the shared part. Let $|*|$ be the Frobenius norm on matrices \cite{}, which is zero only when the matrix whose norm is evaluated is zero. Then, in the appendix we define a certain random variable $X_D$, whose standard deviation $\sigma_d$ and mean $\mu_D$ converge to zero in the limit of dimensions. Then we get that the deviations a random projection which satisfy the following, when $K$ and $D$ tend to infinity in some ratio $\tau>0$,

%\begin{eqnarray*}
%\underbrace{\left|\frac{1}{K} \sum_{k=1}^K Q_{k'}^1(R_i^k - \bar{R}_k)Q_{k'}^1\right|}_{H^k_i = \text{Average deviation}} &\leq& \frac{1}{K}\underbrace{|R_i^{k'} - \bar{R}_{k'}|}_{\text{condition }k'\text{ deviation}} +  \underbrace{\frac{1}{K} \sum_{k \neq k'}  |Q_{k'}^1(R_i^k - \bar{R}_k)Q_{k'}^1|}_{\text{Remaining condition deviations}} %\\
%%&=& \frac{1}{K}|R_i^{k'} - \bar{R}_{k'}| + \frac{1}{K} \sum_{k \neq k'}  |Q_{k'}^i(R_i^k - \bar{R}_k)Q_{k'}^i| \\
%%&\leq& \frac{1}{K}\Gamma + \frac{1}{K} \Gamma \sum_{k \neq k'} X_{k'}
%\end{eqnarray*}

\begin{Prop}
Let $\bar{R_{i}}$ be, as defined in Equation~\ref{eq:av_epoch_cov_classes},
the average condition specific covariance in the $i$-th epoch, $K$ the number of conditions, $N$ the number of epochs, $D$ the number of dimensions, where the number of non-stationary dimensions, $d_n$, is fixed. 

 Assume, that the non-stationarity is bounded, i.e.~for all $i,k$, corresponding to the $i$-th epoch and $k$-th condition, $\vectornorm{R_{i,k} - \frac{1}{N}\sum_{i=1}^NR_{i,k}}_\mathcal{F} < \Gamma$, for some constant $\Gamma$, where $||\cdot||_\mathcal{F}$ is the Frobenius norm on matrices. Assume finally that the columns of the matrices $B_k^\n$, the condition-specific non-stationary subspaces,  are also uniformly distributed with orthonormal columns\footnote{They are a sample of Haar measure.}. 
 
 Then let $P$ be any projection matrix. Then we have the following convergence relation in probability, in $K$ and $D$, of $\bar{R}_i$ to the average covariance over epochs $\frac{1}{N}\sum_{j=1}^N \bar{R}_j$ under the projection $P$, 
 
\begin{multline}
	\text{Pr}\left(\frac{1}{N}\sum_{i=1}^N\vectornorm{P^\top\left( \bar{R_{i}} - \frac{1}{N}\sum_{j=1}^N  \bar{R}_{j}\right)P}_\mathcal{F} \right. \\
\left.	> \mathcal{O}\left(\frac{1}{K}\right) + \mathcal{O}\left(\frac{1}{\sqrt{D}}\right) + \mathcal{O}\left(\frac{1}{\sqrt{\delta \sqrt{D}}}\right)\right) 
		<\delta.
\end{multline}
\label{prop:converge}
\end{Prop}
\begin{proof}
See Appendix \ref{app:proofs}.
\end{proof}

The term on the left of the inequality expresses the non-stationarity
measured in the terms $\bar{R}_i$ over epochs; each term of the sum
expresses the deviation of $\bar{R}_i$ from the average over SSA
epochs.  Note that this is a different measure from the measure of
non-stationarity that we use for \emph{optimization} with SSA: the SSA
objective function is invariant to changes in the parametrization of
the data space, which is desirable for estimation, whereas the measure
in the proposition is not.  However, for the purpose of deriving a
convergence rate, the measure in the proposition is more convient to
use. Nevertheless both measures are equivalent in the sense that each
is zero if and only if the other is zero.

The term on the right of the inequality decreases in $K$ and $D$: for
complete convergence to be guaranteed under the assumptions of the
proposition, note that both $K$ (number of epochs) and $D$ (number of
dimensions) should be assumed to grow. Nevertheless, either $D$ or $K$
increasing guarantee a better estimate. That $D$ may assumed to be
much bigger than $d_n$ in practice is plausible, as often
non-stationarities are confined to low dimensional subspaces, for
example, artifacts in EEG are often confined only to electrodes at the
edge of the scalp.

Note also that the proposition is conditioned on two important assumptions: firstly that the non-stationary subspaces of the condition specific systems are sampled uniformly at random and secondly that 
the non-stationarity is uniformly bounded over classes ($\vectornorm{R_{i,k} - \frac{1}{N}\sum_{i=1}^NR_{i,k}}_\mathcal{F} < \Gamma$).
These are plausible assumptions to make on the model. The first assumption is equivalent to assuming we have no prior knowledge of the condition specific systems's mixing matrices, but may be weakened without making convergence impossible and the second assumption is necessary for estimation to occur at all, but is nevertheless plausible; for example, in the BCI application (below), the condition specific non-stationarities are much weaker than 
the background non-stationarities.
%Under these assumptions it is possible to show, given sufficiently many conditions and stationary directions
%in the condition specific systems, that the algorithm converges to the solution which would have been obtained using SSA in the standard SSA model, as demonstrated in the simulation results displayed in Figure~\ref{fig:acc_sim}.

%The left hand side denotes how much the condition-specific average parameters deviate on an epoch from the time average and the right hand side represents an upper bound
%composed of terms specific to the projected direction and the remaining directions. The second term is a random variable whose mean and variance decreases the
%more condition-specific stationary directions are present. This ensures that we can get as close as necessary to the desired solution.

%\begin{proof}
%\end{proof}

